Projective Limits of State Spaces: Quantum Field Theory without a Vacuum

Instead of formulating the states of a Quantum Field Theory (QFT) as density matrices over a single large Hilbert space, it has been proposed by Kijowski [Kijowski, 1977] to construct them as consistent families of partial density matrices, the latter being defined over small 'building block' Hilbert spaces. In this picture, each small Hilbert space can be physically interpreted as extracting from the full theory specific degrees of freedom. This allows to reduce the quantization of a classical field theory to the quantization of finite-dimensional sub-systems, thus sidestepping some of the common ambiguities (specifically, the issues revolving around the choice of a 'vacuum state'), while obtaining robust and well-controlled quantum states spaces. The present letter provides a self-contained introduction to this formalism, detailing its motivations as well as its relations to other approaches to QFT (such as conventional Fock-like Hilbert spaces, path-integral quantization, and the algebraic formulation). At the same time, it can serve as a reading guide to the series of more in-depth articles [arXiv:1411.3589, arXiv:1411.3590, arXiv:1411.3591, arXiv:1510.01926].

==> meta1.tex <==
\newcommand{\authAffilAbstrac}[1]{\begin{center}\vspace{-0.1cm}%
\Mpar \vspace{\Ssaut}\ensstitre{Suzanne Lanéry}\vspace{0.1cm}%
\Mpar \vspace{\Ssaut}\enmoinsgrand{Centro de Ciencias Matemáticas, Universidad Nacional Autónoma de México, Morelia, México}\vspace{0.2cm}%
\Mpar \vspace{\Ssaut}\makeatletter\@date\makeatother\vspace{-0.4cm}\MsectionBNoNumberNoToc{abstract}{\texorpdfstring{\enssstitre{Abstract}}{Abstract}}\end{center}\vspace{0.3cm}%
\Mpar \vspace{\Ssaut}\enpetit{#1}\vspace{-0.2cm}}


==> meta2.tex <==
\def\Acknowledge{\vspace{-0.7cm}\MsectionBNoNumberNoToc{acknowledgements}{Acknowledgements}\vspace{\PsectionB}%
\Mpar \vspace{\Saut}\hspace{\Alinea}I would like to thank Thomas Thiemann for encouraging me to write this overview letter.%
\Mpar \vspace{\Saut}\hspace{\Alinea}Financial support through the Programa de Becas Posdoctorales de la UNAM is acknowledged.}


==> nota1.tex <==
\RequirePackage{graphicx}\RequirePackage{nicefrac}\RequirePackage{xspace}\newcommand{\mkop}[1]{\mathop{\text{{#1}}}\nolimits}\def\middlewithspace#1{\;\middle#1\;}\newcommand{\longAL}{Ashtekar-Lewandowski\xspace}\newcommand{\extendedLabelSet}{\text{{(ext)}}}

